Human Performance Modeling and Rendering via Neural Animated Mesh

We have recently seen tremendous progress in the neural advances for photo-real human modeling and rendering. However, it's still challenging to integrate them into an existing mesh-based pipeline for downstream applications. In this paper, we present a comprehensive neural approach for high-quality reconstruction, compression, and rendering of human performances from dense multi-view videos. Our core intuition is to bridge the traditional animated mesh workflow with a new class of highly efficient neural techniques. We first introduce a neural surface reconstructor for high-quality surface generation in minutes. It marries the implicit volumetric rendering of the truncated signed distance field (TSDF) with multi-resolution hash encoding. We further propose a hybrid neural tracker to generate animated meshes, which combines explicit non-rigid tracking with implicit dynamic deformation in a self-supervised framework. The former provides the coarse warping back into the canonical space, while the latter implicit one further predicts the displacements using the 4D hash encoding as in our reconstructor. Then, we discuss the rendering schemes using the obtained animated meshes, ranging from dynamic texturing to lumigraph rendering under various bandwidth settings. To strike an intricate balance between quality and bandwidth, we propose a hierarchical solution by first rendering 6 virtual views covering the performer and then conducting occlusion-aware neural texture blending. We demonstrate the efficacy of our approach in a variety of mesh-based applications and photo-realistic free-view experiences on various platforms, i.e., inserting virtual human performances into real environments through mobile AR or immersively watching talent shows with VR headsets.

==> Capture_system.tex <==
\subsection{Background: NeRF and NeuS}\label{sec:capture}

%Since light can be linearly superimposed, given a finite basis set of lighting conditions, we can generate any illumination configuration to the captured target by the superposition approach.
To recover the 4D reflectance fields of dynamic portrait, we build up a light stage device with 96 LED light sources and a stationary 4K ultra-high-speed camera at 1000 fps, resulting in temporal OLAT imageset at 25 fps, so as to provide fine-grained facial perception.

Under such dynamic capture setting, the target performer can freely speak, translate and rotate in a certain range to provide a continuous and dynamic OLAT imagesets sequence. 
%
However, one of the most challenging issue is that the motion of the captured target along with data acquisition will cause mis-alignments, leading to blurriness in the OLAT imagesets, making the data post-processing more challenging. 
%
We conquer such limitations using an optical flow algorithm and further retrieve results at higher frame rate using densely-acquired homogeneous full-lit frames.

\begin{figure}[t]
  \includegraphics[width=\linewidth]{image/capture_settings.png}
  \caption{The demonstration of our capturing system and samples of captured data. Left: cameras and lights are arranged on a spherical structure; (a)-(e): samples of OLAT images; (f) a full-lit frame image. Subfigures on the bottom-left of (a)-(f) illustrates the corresponding lighting conditions on our system.}
  \label{fig:capture_system}
\end{figure}

\subsection{Fast Surface Reconstruction with Hash Encoding}

Our hardware architecture is demonstrated in Fig.~\ref{fig:capture_system}, which is a spherical dome of a radius of 1.3 meters with 96 fully programmable LEDs and a 4K ultra-high-speed camera.
%
The LEDs are independently controlled via a synchronization control system and evenly localized on the doom to provide smooth lighting conditions. 
%
One can simulate any desired environmental map by linearly combining the intensity of 8-bit RGB channels. 
%
Single PCC (Phantom Capture Camera) is leveraged with a global shutter setting, generating roughly 6 TB of data in total. 
%
For each data session, we collect video sequences in 25 seconds rather than isolated frames with 700 us exposure time and 1000 EI, which allows a lower noise floor. 
%
In practice, we can simultaneously control the PCC along with the LEDs system. 
%

\paragraph{Conditioning Feature Maps.}
A conditioning feature maps $\mathbf{F}_t$ consists of a diffuse color image $\mathbf{I}_t^{d}$, a coordinate image $\mathbf{I}_t^{c}$ as well as a landmark image $\mathbf{I}_t^{l}$. 
%
Precisely, the diffuse color image $\mathbf{I}_t^{d}$ and coordinate image $\mathbf{I}_t^{c}$ are rendered from a FLAME~\cite{li2017learning} model of the target actor. 
%
Recall that FLAME~\cite{li2017learning} is a parametric 3D head model described by a function $G(\mathbf{\beta}, \mathbf{\theta}, \mathbf{\phi})$, where the coefficient parameters $\mathbf{\beta}$, $\mathbf{\theta}$, and $\mathbf{\phi}$ represent head shape, head pose and facial expression, respectively. 
%
We adopt an averaged model texture $\mathbf{H}$ of the FLAME dataset as our texture map and render the diffuse color image $\mathbf{I}_t^{d}$ via mesh rasterization with texture mapping and adopt the projected normalized coordinate code (PNCC)~\cite{zhu2017face} to the FLAME model to generate the coordinate image $\mathbf{I}_t^{c}$.
%
These images provide a coarse estimation of the detailed facial geometry and spatial information for result synthesis.
%
However, FLAME model itself can not precisely model fine-grained facial geometry, such as various mouth shapes, leading to a slight misalignment of facial features. 
%
To alleviate such error, we further add a landmark image in $\mathbf{F}_t$ to provide more accurate cues of fine-grained facial geometry and motion. 
%
We adopt the landmark defined as in the approach~\cite{kazemi2014one} and further connect 2D landmark points by segments with semantic meaning and form a landmark image as illustrated in Fig.~\ref{fig:pipeline}.


Given an image of the source actor, we detect a human face and center it in a square region where the face occupies about $65\%$ pixels. 
%
Next, we crop and resize the region from the source image to a uniform size square image patch $\mathbf{I}$. 
%
Face parameters $\mathbf{\beta}$, $\mathbf{\theta}$, and $\mathbf{\phi}$ are extracted from this image patch via the DECA method~\cite{feng2020learning}, while the 2D landmarks are estimated using a regression trees approach~\cite{kazemi2014one}.

\subsection{Surface Rendering}

\paragraph{Semantic Normalization.} 
Note that when the source and target actors are different, their facial geometry will be different even in similar facial expressions, which will manifest in facial characteristics, such as eye size, nose length, mouth curvature, etc., as demonstrated in Fig.~\ref{fig:normalization}.
%
We expect the distribution of conditioning feature maps generated from the source actor is similar to one of the target actor, so as to preserve target-aware appearance rendering results. 
%
To this end, we introduce a semantic-aware facial normalization strategy to the extracted facial parameters and 2D landmarks. 

\begin{figure}[t]
  \includegraphics[width=\linewidth]{image/component_2.png}
  \caption{The illustration of our hierarchical landmark architecture and results before and after the proposed normalization scheme. Left image: black vectors represent the landmark vectors in the first level; Blue vectors in the blue rectangle on the top-right are examples of the ones in the second level. Right image: misalignment of mouth landmark is alleviated after normalization.}
  \label{fig:normalization} 
\end{figure}

Specifically, we assume parameters as random variables which follow the normal distributions. 
%
For each parameter, we normalize both the mean and variance of the source actor's distribution $\mathbf{X}_s\sim N(\mathbf{\mu}_s, \mathbf{\sigma}_s^2)$ to be the same as the target actor's distribution $\mathbf{X}_t\sim N(\mathbf{\mu}_t, \mathbf{\sigma}_t^2)$. 
%
Thus, the normalized parameter $\hat{X}_s$ can be formulated as:
\begin{equation}
\begin{aligned}
\hat{X}_s = (\mathbf{\sigma}_t \oslash \mathbf{\sigma}_s)\circ(\mathbf{X}_s - \mathbf{\mu}_s)+\mathbf{\mu}_t \sim N(\mathbf{\mu}_t, \mathbf{\sigma}_t^2), 
\end{aligned}
\label{eq:normalization}
\end{equation}
where $\oslash$ and $\circ$ are element-wise division and product respectively. 
%
In our implementation, we regard the head pose $\mathbf{\theta}$ and facial expression $\mathbf{\phi}$ of FLAME parameters as two individual random variables and use the Eqn.~\ref{eq:normalization} for normalization.
%
As shown in Fig.~\ref{fig:normalization}, we parameterize the 2D landmark by constructing a two-level hierarchical structure to take both global and local landmark features into account. 
%
In the first level, we group the landmark points of two eyes, two eyebrows, nose, nose bridge and mouth into seven clusters according to their categories. 
%
The root point is defined as the center of all landmark points.
%
Then, the root point and the cluster centers form landmark vectors $\{\mathbf{l}_{1,i}\}_{i=1}^7$ of the first level, which represent the global spatial information of the face. 
%
In the second level, each cluster center with landmark points inside the cluster forms landmark vectors $\{\mathbf{l}_{2,i}^j\}_{j=1}^{n_i}$ of the second level for $i$-th category, where $n_i$ is the number of landmark points in category $i$. 
%
The second level landmark vectors record the local arrangement of landmark points inside clusters, which will provide more accurate descriptions of facial features compared to FLAME model. 
%
We regard each landmark vector from all the levels as a random variable and normalize them according to Eqn.~\ref{eq:normalization}. 
%
Then, a normalized 2D landmark image $\mathbf{\tilde{I}}_t^l$ is reconstructed using these normalized landmark vectors in such a hierarchical manner.
%
Thus, the conditioning feature maps $\mathbf{F}_t$ at time $t$ are formulated as:
\begin{equation}
\begin{aligned}
\mathbf{F}_t = \{\mathbf{\tilde{I}}_t^{d}, \mathbf{\tilde{I}}_t^{c}, \mathbf{\tilde{I}}_t^{l}\},
\end{aligned}
\label{eq:conditioning_feature}
\end{equation}
where $\mathbf{\tilde{I}}_t^{d}, \mathbf{\tilde{I}}_t^{c} = \Pi(G(\mathbf{\beta}, \mathbf{\tilde{\theta}}, \mathbf{\tilde{\phi}}), \mathbf{H})$ and $\Pi$ is the rasterization and texture mapping function; $\mathbf{\tilde{\theta}}$ and $\mathbf{\tilde{\phi}}$ are normalized parameters.


